Top-k Connected Overlapping Densest Subgraphs in Dual Networks

Networks are largely used for modelling and analysing data and relations among them. Recently, it has been shown that the use of a single network may not be the optimal choice, since a single network may misses some aspects. Consequently, it has been proposed to use a pair of networks to better model all the aspects, and the main approach is referred to as dual networks (DNs). DNs are two related graphs (one weighted, the other unweighted) that share the same set of vertices and two different edge sets. In DNs is often interesting to extract common subgraphs among the two networks that are maximally dense in the conceptual network and connected in the physical one. The simplest instance of this problem is finding a common densest connected subgraph (DCS), while we here focus on the detection of the Top-k Densest Connected subgraphs, i.e. a set k subgraphs having the largest density in the conceptual network which are also connected in the physical network. We formalise the problem and then we propose a heuristic to find a solution, since the problem is computationally hard. A set of experiments on synthetic and real networks is also presented to support our approach.

==> name.tex <==
\begin{algorithm}[hp!]
\SetAlgoLined
\KwResult{Accept or Refuse the $H_0$ hypothesis}
 {Let $S_{gi}$ a given solution }\;
 {Let $SS(S_{gi})$ its internal semantic similarity}\;
 {Let $V_s$ the set of 100 random solutions $V_s$=\{$RS_{j}$\}} j=0,..,99;\\
 \ForEach{$RS_{j} \in V_s$}
   {calculate $SS_j(RS_{j})$ the internal semantic similarity of each random solution}\;
 {Compare $SS(S_{gi})$  and all the $SS_j(RS_{j})$ using a non parametric test}\;
 {Accept or Refuse the Hypothesis $SS(S_{gi})$ is significantly higher than $SS_j(RS_{j})$}\;
\caption{Biological Evaluation of Results}
\label{algo:rel}
\end{algorithm}
